Complete Test Sets And Their Approximations

We use testing to check if a combinational circuit $N$ always evaluates to 0 (written as $N \equiv 0$). We call a set of tests proving $N \equiv 0$ a complete test set (CTS). The conventional point of view is that to prove $N \equiv 0$ one has to generate a trivial CTS. It consists of all $2^{|X|}$ input assignments where $X$ is the set of input variables of $N$. We use the notion of a Stable Set of Assignments (SSA) to show that one can build a non-trivial CTS consisting of less than $2^{|X|}$ tests. Given an unsatisfiable CNF formula $H(W)$, an SSA of $H$ is a set of assignments to $W$ that proves unsatisfiability of $H$. A trivial SSA is the set of all $2^{|W|}$ assignments to $W$. Importantly, real-life formulas can have non-trivial SSAs that are much smaller than $2^{|W|}$. In general, construction of even non-trivial CTSs is inefficient. We describe a much more efficient approach where tests are extracted from an SSA built for a `projection' of $N$ on a subset of variables of $N$. These tests can be viewed as an approximation of a CTS for $N$. We give experimental results and describe potential applications of this approach.

==> f8ootnote.tex <==
Informally, property $\xi_i$ of $M$ is ``local'' if only a fraction of
$M$ is responsible for $\xi_i$.


==> f9ootnote.tex <==
\label{foot:loc_prop}
Let $N$ be the circuit obtained by composing $M_T$ and a $|C|$-input
AND gate representing the negation of $C$. Then $N$ evaluates to 1 iff
the output of $M_T$ falsifies $C$. Proving $P(S) \wedge T \rightarrow
C(S')$ reduces to showing that $N \equiv 0$ for every input assignment
satisfying $P$. This is a variation of the problem we consider in this
paper (i.e. checking if $N \equiv 0$ holds). Fortunately, this
variation of the original problem can be solved by \sas.



==> junk.tex <==

\vspace{20pt}

just something to fill out the page
\clearpage
just something to fill out the page
\clearpage


==> s0torage.tex <==
Otherwise, according to definitions of
Subsection~\ref{ssec:approx}, if $X \subseteq V$ (respectively $X
\not\subseteq V$), \ti{GenPCT} generates a \acts (respectively
\aacts).
-------
In this section, we describe experiments with property-checking tests
(PCT) generated by procedure \ti{GenPCT} shown in
Figure~\ref{fig:gen_pct}. Given a single-output circuit $N$,
\ti{GenPCT} starts with generating formula $F_N \wedge z$ and a set of
variables $V \subseteq \V{F_N \wedge z}$. Then it calls \sas (see
Fig.~\ref{fig:sem_str}) to compute an SSA $P$ of formula $H(V)$
describing a projection of circuit $N$ on $V$. If $H(V)$ does not
depend on a variable $w \in V$, all assignments of $P$ have the same
value of $w$. Procedure \ti{Diversify} randomizes the value of $w$ in
the assignments of $P$.
----------
Building an SSA for a large formula is inefficient. So, constructing
  a CTS of $N$ from an SSA of $F_N \wedge z$ is impractical. To
  address this problem, we introduce a procedure called \sas (a short
  for ``Semantics and Structure''). Given formula $G$ and a set of
  variables $V \subseteq \V{G}$, \sas generates a simpler formula
  $H(V)$ implied by $G$ at the same time trying to build an SSA for
  $H$. If \sas succeeds in constructing an SSA of $H$, the latter is
  unsatisfiable and so is $G$.

  \sas can be applied to $F_N \wedge z$ to generate tests as
  follows. Let $V$ be a subset of \V{F_N \wedge z}. First, \sas
  constructs a formula $H(V)$ implied by $F_N \wedge z$ and an SSA of
  $H$. Then a set of tests $T$ is extracted from this SSA. As we show
  in Subsection~\ref{ssec:approx}, one can view $T$ as an
  approximation of a CTS for $N$ (if $X \subseteq V$) or an
  ``approximation of approximation'' of a CTS (if $X \not\subseteq
  V$).
-------------
Implication $G \rightarrow H$ is a \ti{semantic} property of $G$.  To
verify this property it suffices to know the truth table of $G$.
-----------
We will refer to the procedure that proves unsatisfiability of $F_N
  \wedge z$ by building formula $H$ and its SSA as \sas
  (``\ti{Sem}antics and \ti{Str}ucture'').
  ------------
Here are some reasons why such tests can be very
  useful.
  ---------
The latter is a special case of an incomplete/incorrect
design specification.
---------
The latter is a
\ti{weaker} property than regular one, which should cause problems for
traditional testing. (Arguably, the conventional methods of testing
favor breaking strong properties over weak ones).
------
%
\begin{corollary}
  Let $P$ be an SSA of $H$ with respect to PC-mapping \Fi.
  Then the set of clauses \ac{P} is unsatisfiable. Thus,
  every clause of $H \setminus \ac{P}$ is redundant.
\end{corollary}
----------
Note that if $P$ is an SSA of $H$ with respect to AC-mapping \Fi, it
is an SSA of \ac{P} as well.
--------------
There are many reasons for
  property-checking test sets to be extremely useful.  Here is one of
  them.  Let $\Xi :=\s{\xi_1,\dots,\xi_k}$ be the set of properties of
  $M$ formulated by the designer. Assume that $\Xi$ is incomplete
  (i.e. the fact that every $\xi_i \in \Xi$ holds does not imply that
  $M$ is correct).  Then a test for which every $\xi_i \in \Xi$ holds
  can still expose a bug (breaking a missed property of $M$). So, if
  $M$ \ti{does not fail} on tests generated for the properties of
  $\Xi$, one gets extra guarantee that $M$ is correct.
  -----------------
Procedure \ti{GenCls} is shown in Figure~\ref{fig:gen_cls}. First,
\ti{GenCls} checks if formula $G$ is satisfiable under assignment
\pnt{v}.  If so, an assignment \pnt{s} satisfying $G$ is
returned. Otherwise, a proof $R$ of unsatisfiability is returned by
\ti{ChkSat}.  Then \ti{GenCls} forms the subset $G'$ of clauses of $G$
used in proof $R$ that contain variables of $V$. (All clauses of $G'$
with a variable of $V$ have the same literal of this variable
falsified by \pnt{v}). The literals of $V$ present in clauses of $G'$
specify a clause $C$ that is implied by $G$ and falsified by \pnt{v}.
----------
%
% Gen Clause
%

\begin{wrapfigure}{L}{1.4in}
%\begin{center}
\small

\begin{tabbing}
aa\=bb\=cc\= dd\= \kill
$\mi{GenCls}(G,V,\pnt{v})$\{\\
\tb{\scriptsize{1}}\> $(\pnt{s},R) := \mi{ChkSat}(G,\pnt{v})$\\
\tb{\scriptsize{2}}\> if ($\pnt{s} \neq \mi{nil}$) return($\mi{nil},\pnt{s}$)\\
\tb{\scriptsize{3}}\> $G' := \mi{Analyze}(R,G,V)$\\
\tb{\scriptsize{4}}\> $C := FormCls(G',V)$ \\
\tb{\scriptsize{5}}\>  return($C,\mi{nil}$)\\
\end{tabbing} 
\vspace{-15pt}
\caption{\ti{GenCls} procedure}
%\vspace{5pt}
\label{fig:gen_cls}
\end{wrapfigure}
%\end{figure}
---------
The fact
that there always exists at least one cut $R$ where $N_R$ is
non-redundant eliminates degenerate single-test CTSs for $N$.
------------
So a solution to the problem caused by redundancy of $N$ is as
follows.  One should require that for every cut $R$ where $N_R \equiv
0$ holds, set $T_R \cup T^*_R$ should be a CTS for $N_R$. The fact
that there always exists at least one cut $R$ where $N_R$ is
non-redundant eliminates degenerate single-test CTSs for $N$.
----------------
Assume the contrary. Let $P$ be an SSA of $H$ with
center \sub{p}{init} and AC-mapping \Fi and $H$ is
satisfiable. Let \pnt{s} be an assignment satisfying $H$. Let \pnt{p}
be an assignment of $P$ that is the closest to \pnt{s}~\,in terms of
the Hamming distance.  Let $C = \Fi(\pnt{p})$. Since \pnt{s} satisfies
clause $C$, there is a variable $v \in \V{C}$ that is assigned
differently in \pnt{p} and \pnt{s}.  Let \pnt{p^*} be the assignment
obtained from \pnt{p} by flipping the value of $v$.  Note that
$\pnt{p^*} \in \mi{Nbhd}(\sub{p}{init},\pnt{p},C)$.

Assume that $\pnt{p^*} \in P$. In this case, \pnt{p^*} is closer
to \pnt{s} than \pnt{p} and we have a contradiction. Now, assume that
$\pnt{p^*} \not\in P$. In this case,
$\mi{Nbhd}(\sub{p}{init},\pnt{p},C) \not\subseteq P$ and so set $P$ is
not an SSA. We again have a contradiction.
----------
The proof is given in~\cite{cmpl_tst}. A similar proposition was
proved in~\cite{ssp} for ``uncentered'' SSAs (see
Footnote~\ref{ftn:ssa}).
------------
A flaw of this approach is
that testing is treated as a second-class citizen whose quality can be
measured only by a formal proof it encodes.
------------
To make property \pim even
``weaker'' and so harder for traditional methods of testing, we
modified $M$ so that the two circuits feeding outputs of $M$ were
independent of each other. (This was done by duplicating gates shared
by both circuits.)
-----------------------
Importantly, a formal tool may
miss this bug since it does not break property $\xi$.
-----------
(This procedure is non-deterministic: an
oracle is used in line 7 to pick the variable to flip.)
----------------
We will refer to the procedure that proves unsatisfiability of $F_N
  \wedge z$ by building formula $H$ and its SSA as \sas
  (``\ti{Sem}antics and \ti{Str}ucture'').  \sas can be applied to an
  arbitrary CNF formula $G(V,W)$. If $G$ is unsatisfiable, \sas
  returns a formula $H(V)$ implied by $G$ and its SSA. Otherwise, it
  produces an assignment to $V \cup W$ satisfying $G$.  \sas combines
  semantic and structural derivations. The semantic part of \sas
  is\footnote{\input{f6ootnote}} to derive $H$. Its structural part
  consists of proving that $H$ is unsatisfiable by constructing an
  SSA.
  ---------
The contribution of this paper is fourfold. First, we use the
  machinery of SSAs to introduce the notion of non-trivial CTSs
  (Section~\ref{sec:cts}). Second, we present \sas, a key procedure
  for efficient construction of approximations of CTS
  (Sections~\ref{sec:algor} and~\ref{sec:app_cts}).  Third, we
  describe some applications of such tests (Section~\ref{sec:appl}).
  Fourth, we give experimental results showing the effectiveness of
  tests produced by \sas (Section~\ref{sec:exper}).
--------------

Term CTS is sometimes used to say that a test set is complete in terms
of a \ti{coverage metric} i.e. that every event considered by this
metric is tested. Our application of term CTS is obviously quite
different.
---------
If $X \subseteq V$, the
projection of $N$ on $V$ is of the first kind. Otherwise, it is a
projection of the second kind.
-----------
Property \pim requries only that for every input
assignment at least one output of $M$ and $M^{\pi}$ produces the same
value.
--------
%
%
%\vspace{-5pt}
%\begin{wraptable}{L}{2.9in}
\begin{table}
\small
\caption{\ti{Testing corner cases}}
\vspace{-5pt}
\scriptsize
\begin{center}
%\renewcommand{\arraystretch}{1.2} % Default value: 1
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
\begin{tabular}{|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|} \hline
~~name          &la- & \#inp &\#and &\,\#ga- & \multicolumn{3}{c|}{random} & \multicolumn{4}{c|}{testing by}  \\
                &tch&  vars   &vars &\,tes  & \multicolumn{3}{c|}{testing} & \multicolumn{4}{c|}{\acts and \aacts}  \\ \cline{6-12}
                &     &    &     &      &\,\#te-\,   &\,\#hits\,& \,time\, &\,test\,&~\#te- &\,\#hits\,  &~time\,  \\ 
                &     &    &     &      &\,sts\,     & ~\%    &~(s.)      &\,set\,&~sts   &~ \%      &~(s.) \\ \hline
  pd..gigamax5  & L46 & 43 & 10  &\,512\,  &\,$10^5$\,&~0.02  &~2.0    &\,\tiny{\acts}&~547   &~7.1   & ~0.2   \rule{0pt}{2.8mm}     \\ \hline
  pd..gigamax5  & L46 & 63 & 30  &\,512\,  &\,$10^7$\,&~0     &~218    & \,\tiny{\acts} &~1,243\,   &~3.0    &~ 0.2     \rule{0pt}{2.8mm}     \\ \hline
  pdtvisbpb1    & L48 & 46 & 10  &\,108\, &  $10^5$   &~0.04   &~0.7   & \,\tiny{\acts} &~398      &~9.0   &~0.01 \rule{0pt}{2.8mm}            \\ \hline
  pdtvisbpb1     & L48 & 66 & 30  &\,108\, &  $10^7$   &~0     &~78    & \,\tiny{\acts} &~736      &~3.1    &~0.03 \rule{0pt}{2.8mm}            \\ \hline
   abp4pold      &L270 & 139  & 10  &\,637\, & $10^5$  &~0.02  &~3.8   & \,\tiny{\aacts} &~3,725    &~7.8    &~1.5  \rule{0pt}{2.8mm}            \\ \hline
    abp4pold     &L270 & 159  & 30  &\,637\,& $10^7$   &~0     &~399   & \,\tiny{\aacts} &~9,692    &~3.1    &~3.4  \rule{0pt}{2.8mm}            \\ \hline
mentorbm1p00  &  L8670 &636  & 10 &\,1,630\, & $10^5$ &~0.1    &~8.4   & \,\tiny{\aacts} &~1,619    &~15     &~6.2 \rule{0pt}{2.8mm}            \\ \hline
mentorbm1p00   & L8670 &656  & 30 &\,1,630\, & $10^7$ &~0      &~876   & \,\tiny{\aacts} &~2,473    &~7.9    &~5.3 \rule{0pt}{2.8mm}            \\ \hline
%   &     &    &  &    &        &            &         &               &    &         &   \rule{0pt}{2.8mm}            \\ \hline
\end{tabular}                
\end{center}
\vspace{-20pt}
\label{tbl:corners}
\end{table}
%\end{wraptable}


We use relaxed equivalence checking to show that
traditional testing can have problems with verifying
\ti{weak} properties.
---------
This CTS was
obtained by applying \sas to formula $F_N \wedge z$ with an empty set
of variables to exclude. In this case, the resulting formula $H$ is
equal to $F_N \wedge z$ and \sas just constructs its SSA.
---------
Subsection ~\ref{ssec:cts}
compares CTSs, \acts{s} and \aacts{s}.  In Subsection~\ref{ssec:bug},
we show that re-using \aacts{s} can be effective in bug detection.  In
Subsection~\ref{ssec:ecorners}, \acts{s} and \aacts{s} are used to
increase frequency of hitting corner cases. Finally,
Subsection~\ref{ssec:missed_props} demonstrates that property-checking
tests can be used for breaking a ``missed'' property.
----------
We will refer to $W$ as the set of variables to
 \ti{exclude}.
 ------------
% SemStr
\begin{wrapfigure}{L}{1.8in}
%\begin{center}
\small
%\normalsize
\vspace{-5pt}
\begin{tabbing}
aa\=bb\=cc\= dd\= \kill
$\mi{SemStr}(G,(V,W))$\{\\
\tb{\scriptsize{1}}\> $H := \emptyset$ \\
\tb{\scriptsize{2}}\> while (\ti{true}) \{ \\
\tb{\scriptsize{3}}\Tt $(\pnt{v},\!P,\!\sub{p}{init},\!\Fi)\!:=\!\mi{BuildSSA}(H)$\\
\tb{\scriptsize{4}}\Tt if ($P \neq \mi{nil}$)  \\
\tb{\scriptsize{5}}\ttt return($\mi{nil},H,P,\sub{p}{init},\Fi$)\\
\tb{\scriptsize{6}}\Tt  $(C,\pnt{p}) := \mi{GenClause}(G,V,\pnt{v})$ \\
\tb{\scriptsize{7}}\Tt  if ($\pnt{p} \neq \mi{nil}$) \\
\tb{\scriptsize{8}}\ttt return($\pnt{p},\mi{nil},\mi{nil},\mi{nil},\mi{nil}$)\\
\tb{\scriptsize{9}}\Tt  $H := H \cup \s{C}$ \} \\
\end{tabbing} 
\vspace{-20pt}
\caption{\ti{SemStr} procedure}
\label{fig:sem_str}
\end{wrapfigure}
%\end{figure}
----------
In the first three experiments, we used miters i.e. circuits
specifying the property of equivalence checking (see
Figure~\ref{fig:gen_miter}).  In the fourth experiment, we applied our
approach to circuits generated in Bounded Model Checking
(BMC)~\cite{bmc}.  In Section~\ref{sec:app_cts} we described an
autonomous procedure \ti{GenTests} for building a test set. For the
sake of simplicity, we assume here that \ti{GenTests} is incorporated
into \sas.
------------
The pseudocode of \sas is shown in Figure~\ref{fig:sem_str}.  \sas
accepts formula $G(V,W)$ and generates an assignment satisfying $G$ or
formula $H(V)$ implied by $G$ and an SSA of $H$.  Originally set of
clauses $H$ is empty. $H$ is computed in a while loop. First, \sas
looks for an assignemnt \pnt{v} satisfying $H$ (line 3).  If $H$ is
unsatisfiable, \sas computes its SSA and returns this SSA and $H$
(lines 4-5). Otherwise, \sas calls procedure \ti{GenClause} to build a
clause $C$ falsified by \pnt{v}.  Clause $C$ is obtained by resolving
clauses of $G$ on variables of $W$. (Hence $C$ is implied by $G$.)  If
\pnt{v} can be extended to an assignment \pnt{p} satisfying $G$, then
\sas terminates (line 9). Othwerwise, $C$ is added to $H$ and a new
iteration begins.
------------
The contribution of this paper is threefold. First, we use the
  machinery of SSAs to introduce the notion of non-trivial CTSs
  (Section~\ref{sec:cts}). Second, we present \sas, a SAT-algorithm
  that combines structural and semantic derivations
  (Section~\ref{sec:algor}).  We show that this algorithm can be used
  for computing a CTS for a projection of a circuit.  We also discuss
  some applications of \sas (Section~\ref{sec:appl}).  Third, we give
  experimental results showing the effectiveness of tests produced by
  \sas (Section~\ref{sec:exper}).
 ----------
%
% SemStr
%
%\setlength{\intextsep}{5pt}
%\setlength{\textfloatsep}{10pt}
%\begin{figure}
\begin{wrapfigure}{L}{1.8in}
%\begin{center}
\small
%\normalsize
\vspace{-5pt}
\begin{tabbing}
aa\=bb\=cc\= dd\= \kill
$\mi{SemStr}(G(V,W))$\{\\
\tb{\scriptsize{1}}\> $H := \emptyset$ \\
\tb{\scriptsize{2}}\> while (\ti{true}) \{ \\
\tb{\scriptsize{3}}\Tt $\pnt{v} := CheckSat(H)$ \\
\tb{\scriptsize{4}}\Tt if ($\pnt{v} = \mi{nil}$) \{ \\
\tb{\scriptsize{5}}\ttt $(P,\sub{p}{init},\Fi) := \mi{BldSSA}(H)$\\
\tb{\scriptsize{6}}\ttt return($\mi{nil},H,P,\sub{p}{init},\Fi$)\}\\
\tb{\scriptsize{7}}\Tt  $(C,\pnt{p}) := \mi{GenClause}(G,V,\pnt{v})$ \\
\tb{\scriptsize{8}}\Tt  if ($\pnt{p} \neq \mi{nil}$) \\
\tb{\scriptsize{9}}\ttt return($\pnt{p},\mi{nil},\mi{nil},\mi{nil},\mi{nil}$)\\
\tb{\scriptsize{10}}\Tt  $H := H \cup \s{C}$ \} \\
\end{tabbing} 
\vspace{-20pt}
\caption{\ti{SemStr} procedure}
\label{fig:sem_str}
\end{wrapfigure}
%\end{figure}
--------------
In this paper, we give
  two more reasons for generation of PCT. Namely, we show that PCT can
  be used to verify design changes and increase the frequency of
  hitting ``corner cases''.
  ----------------
(In experiments, $F_N \wedge z$ was relaxed as
follows. First, one randomly picked a variable of $F_N \wedge z$. Then
the clauses containing this variable were removed from $F_N \wedge
z$.)
---------%
%
%\vspace{-5pt}
\begin{wraptable}{l}{2.2in}
%\begin{table}
\small
\caption{\ti{Testing a ``missed'' property of a counter}}
\vspace{-5pt}
\scriptsize
%\begin{center}
%\renewcommand{\arraystretch}{1.2} % Default value: 1
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|} \hline
           &\,\#time\,  & \multicolumn{3}{c|}{random testing} & \multicolumn{5}{c|}{testing}  \\
  ~$C_n$~  &\,fra-& \multicolumn{3}{c|}{} & \multicolumn{5}{c|}{by \aacts}  \\ \cline{3-10}
      &\,mes  &\,\#tests\,   &\,suc-\,& \,time\, &\,$|V|$\,&\,\#it\,& \,\#te- &\,suc-\,  &\,time\,  \\ 
      &      &$\times 10^6$ &\,sess\,&~(s.) & &\,ter & \,sts\,  &\,sess\,&~(s.) \\ \hline
$\,C_4$  &~14   &\,0.001         &   \,yes\,     &  ~0~      &\,14&\,1 & \,572\,  &\,yes\, & \,0.1 \rule{0pt}{2.8mm}    \\ \hline
$\,C_5$  &~30   &\,28\,&\,yes\,        & \,363\,     &\,14&\,2 & \,1,393\,  &\,yes\, & \,0.2  \rule{0pt}{2.8mm}   \\ \hline
$\,C_6$  &~62    &\,100        &\,no\,         &  \,4,215\,  &\,14\,&\,2 &\,338\,  &\,yes\, &\,0.5   \rule{0pt}{2.8mm}            \\ \hline
$\,C_7$  &~126   &\,100  &   \,no\,           & \,15,538\,  &\,14\,&\,1 &\,1,025\,  &\,yes\, &\,2.1   \rule{0pt}{2.8mm}            \\ \hline
%     &       &        &            &         &  & &                   &         &   \rule{0pt}{2.8mm}            \\ \hline
\end{tabular}                
%\end{center}
%\vspace{-5pt}
\label{tbl:missed}
%\end{table}
\end{wraptable}
------
%
%
%\vspace{-5pt}
\begin{table}
%\begin{wraptable}{l}{2.65in}
\small
\caption{\ti{Computing CTSs, \acts{s} and \aacts{s}}}
\vspace{-5pt}
\scriptsize
\begin{center}
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
\begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{\,}|@{\,}l@{}|@{\,}l@{~}|@{~}l@{~}|} \hline
~name     & \,la- &\,\#inp\,&\,\#ga-   & \multicolumn{2}{c|}{CTS  } & \multicolumn{4}{c|}{\acts or \aacts }  \\ \cline{5-10}
         &\,tch  &\,vars\,&\,tes          &\,\#SSA &\,time\,  &\,test\,&  & \#SSA   &  time  \\ 
  &       &         &           &\,(\#tsts)&~(s.) &\,set\, & \,$|V|$\,  &(\#tsts)   & (s.) \\
   &       &         &           &~$\times 10^3$ &       &       &       & $\times 10^3$  &        \\ \hline
\,bob3 &  \,L26  & \,14    &\,41     &\,46~(2.0)    &\,0.1         &\,\tiny{\acts}  &\,14  &\,0.6    & 0.01  \\ \hline
\,eijks258   &  \,L10  & \,16    &\,45     &\,259~(8.2)&\,0.5    &\,\tiny{\acts}  &\,16  &\,0.1   & 0.02 \\ \hline
\,cmudme1    &  \,L230 &  \,19    & \,50     &\,2,184~(63)\, &\,5.4     &\,\tiny{\acts} &\,19  &\,13 & 0.1 \\ \hline
\,mutexp0    &\,L60  & \,29    & \,199    &  ~memout   & ~$*$    &\,\tiny{\acts}&\,29  & 659 &\,26 \\ \hline
\,pdtpmsmiim\, &\,L118  & \,31    & \,136    &  ~memout  & ~$*$   & \,\tiny{\acts} &\,31  &\,936 & 4.2 \\ \hline
\,abp4pold   &\,L270  &\,129    & \,1,178\,&  ~memout  & ~$*$   &\,\tiny{\aacts}\,&\,28   &\,5.0~(1.0)\, & 0.4  \\ \hline
\,pj2009  &\,L1318\,&\,366     & \,25,160\,& ~memout   & ~$*$   & \,\tiny{\aacts}\,   &\,28 &\,2.7~(1.1)\, & 38 \\ \hline
\,mentorb..00  &\,L8670\,&\,626 &\,3,156\, & ~memout    & ~$*$   &\,\tiny{\aacts}\,    &\,31 &\,12~(3.5)\, & 6.1 \\ \hline
\,139454p0&\,L1676\,&\,791     &\,19,843\,& ~memout  & ~$*$   & \,\tiny{\aacts}\,  &\,24  &\,0.2~(0.1)\,  & 64 \\ \hline
%  &       &         &           &                           &        &     &&      &  \\ \hline
\end{tabular}                
\end{center}
\vspace{-5pt}
\label{tbl:cts}
%\end{wraptable}
\end{table}
---------
A big
advantage of the uncentered SSA though is that its definition
facilitates computing an SSA in clusters of assignments (rather than
single assignments).
----------
%
%
%\vspace{-5pt}
\begin{table}
%\begin{wraptable}{l}{2.65in}
\small
\caption{\ti{Bug detection. \aacts{s} are computed for $|V|=18$. The number of random
tests is limited to $10^8$. An asterisk marks a run where a bug is found.}}
\vspace{-5pt}
\scriptsize
\begin{center}
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
  \begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|} \hline
~name     &\,la- &\,\#inp\,&\,\#ga-   & \multicolumn{2}{c|}{SAF} &  \multicolumn{2}{c|}{random} & \multicolumn{3}{c|}{testing by }  \\
         &\,tch &\,vars\,&\,tes      & \multicolumn{2}{c|}{tests} & \multicolumn{2}{c|}{tests} &\multicolumn{3}{c|}{\aacts}  \\ \cline{5-11}
         &     &       &    &\,\#tests\,& \,time\,&~~\#tests\,&\,time\,&\,\#SSA\,&\,\#tests\,&\,time\, \rule{0pt}{2.8mm} \\ 
&       &         &            &  & ~(s.) & &~(s.)& & &~(s.) \\ \hline
\,cmugigamax       &\,L124\,&\,104 &\,2,007\,   &\,989    &\,4.5  &~~$10^8$ &\,1,649\,&~50   &\,3,421 &\,22$^*$  \rule{0pt}{2.8mm}\\ \hline
\,kenoopp1         &\,L198\,&\,162 &\,2,247\,  &\,1,007  &\,4.7  &~~$10^8$&\,2,147\,  &~72  &\,2,345   &\,20$^*$  \rule{0pt}{2.8mm} \\ \hline
\,pd..ackjack4\,&\,L120\,&\,198 &\,1,251\,  &\,  216  &\,0.4   &\,2,441,892\,&~30$^*$\,  &~62   &\,728     &\,8.5\rule{0pt}{2.8mm}\\ \hline
\,pdtpmsns2        &\,L56 \,&\,236 &\,1,187\,  &\,967    &\,1.0  &~~$10^8$ &\,1,507\,&~31 &\,560&\,1.2$^*$ \rule{0pt}{2.8mm}\\ \hline
\,abp4pold         &\,L270\,&\,258 &\,2,547\,   &\,1,306   &\,6.6 &~~$10^8$ &\,3,555\,&~22 &\,500 &\,1.5$^*$  \rule{0pt}{2.8mm}\\ \hline
\,pdtvissfeistel\,&\,L604\,&\,342 &\,2,111\,   &\,1,232   &\,2.8 &~~$10^8$&\,4,557\,&~86  &\,932       &\,35$^*$ \rule{0pt}{2.8mm}\\ \hline
% \,kenflashp03     &\,L200\,&\,180 &\,14,943\,  &\,        &\,   &&       &\,      &\,        &\,    \rule{0pt}{2.8mm}\\ \hline
\,neclaftp1001    &\,L958\,&\,398 &\,2,707\,  &\,1,723       &\,0.2    &~~$10^8$&1,313&~40    &\,417    &\,6.7$^*$ \rule{0pt}{2.8mm}\\ \hline
\,mentorb..00\,   &\,L8158\,&\,640&\,2.951\, &\,1,932   &\,10  \,&\,3,412,894\,&\,688$^*$\,&~43 &\,1,476 &\,15$^*$    \rule{0pt}{2.8mm}\\ \hline
%\,                 &\,    \,&\,    &\,     \,  &\,        &\,        &&  &\,      &\,       &\,    \rule{0pt}{2.8mm}\\ \hline
\end{tabular}                
\end{center}
\vspace{-5pt}
\label{tbl:flt_tst}
%\end{wraptable}
\end{table}
-------
The first column of
the four gives the size of set $V$ specifying an internal cut of $N$
picked as described in Subsection~\ref{ssec:int_cut}. The next two
columns show the size of SSA for formula $H(V)$ generated by \sas and
that of test set extracted from this SSA. The fourth column of gives
the number of countexamples. The last column shows the total run-time
that consists of the time taken by \sas to generate $T$ and the time
taken by Minisat to run tests.
------------
We compared our approach with random testing. Our objective was to
show that even \aacts (that is far from being complete) is quite
\ti{effective}. Every bug that was easy for random testing was also
easy for our approach. In Table~\ref{tbl:flt_tst}, we list some
examples that turned out to be hard for random testing.
----------
In the second experiment, we checked the idea of
Subsection~\ref{ssec:des_changes} of re-using test sets to make sure
that a property holds after a design change. More specifically, we
checked that a design change does not change the functionality of a
circuit.  Let $N$ be the miter of circuits $M'$ and $M''$ where $M''$
is just a copy of $M'$. Obviously, $N \equiv 0$ holds. Let $N^*$
denote the miter of circuits $M'$ and $M''$ where $M''$ is obtained
from $M'$ by introducing a change making $M'$ and $M''$ inequivalent.
To check if $N^* \equiv 0$ holds we ran a \aacts generated when
proving $N \equiv 0$.
----------
\subsection{Verification of design changes}
\label{ssec:des_changes}

%
\input{s3ubcirc.fig}
%

Let $\xi$ be a property $M$ specified by circuit $N$.  Let $T$ be PCT
generated when proving that $N \equiv 0$. Suppose that $M^*$ is
obtained from $M$ by a design change. Consider the following two
scenarios in which $T$ can be very useful in testing $M^*$. The first
scenario is that $\xi$ is supposed to hold for $M^*$. Then one can
apply $T$ to circuit $N^*$ specifying property $\xi$ for $M^*$.  Since
$T$ was generated for testing the same property for a close circuit
$M$, there is a good chance it will break $\xi$ if $M^*$ is
incorrect. (Of course, the fact that $N^*$ evaluats to 0 for all tests
of $T$ does not mean that $N^* \equiv 0$ even if $T$ is a CTS for
$N$). Assuming that $\xi$ was proved formally for $M$, this property
can be formally verified for $M*$ too. So, in this scenario, running
$T$ can be viewed as a ``light'' verification procedure for exposing
bugs.



The second scenario is that the designer decides that $M^*$ does not
need property $\xi$. Then running $T$ on $M^*$ can be useful for the
following reason. Suppose $M^*$ is a part of a large design $D$.  By
running $T$ on $M^*$ one produces output assignments breaking $\xi$.
If dropping property $\xi$ is wrong, these output assignments can
expose a bug in design $D$. Note that exposing such a bug by a formal
tool may be impossible if $D$ is too large.
------
\small
\caption{\ti{Bug detection}}
\vspace{-5pt}
\scriptsize
\begin{center}
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
  \begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|} \hline
~name     &\,la- &\,\#inp\,&\,\#ga-   & \multicolumn{3}{c|}{tests detecting} & \multicolumn{5}{c|}{testing by }  \\
         &\,tch &\,vars\,&\,tes      & \multicolumn{3}{c|}{stuck-at faults} & \multicolumn{5}{c|}{\aacts}  \\ \cline{5-12}
         &     &       &    &\,\#tests\,&\,\#cex\,     &\,time     &\,$|V|$\,&\,\#SSA\,&\,\#tests\,&\,\#cex\,&\,time\, \rule{0pt}{2.8mm} \\ 
&       &         &            &  &  &~(s.) & &   &   & &~(s.) \\ \hline
\,cmugigamax       &\,L124\,&\,104 &\,2,007\,   &\,989   &~0  &\, 3.2     &~24   &\, 54   &\,1,387  &\, 1 &\,7.3\\ \hline
\,kenoopp1         &\,L198\,&\,162 &\,2,247\,  &\,1,007  &~0  &\, 3.5  &~20    &\,  60  &\,2,158 &\,  1  &\,42  \rule{0pt}{2.8mm} \\ \hline
%\,pd..blackjack4   &\,L120\,&\,198 &\,1,251\,  &\,       &~0  &\,      &~      &\,      &\,      &\,    &\,    \rule{0pt}{2.8mm}\\ \hline
\,pdtpmsns2        &\,L56 \,&\,236 &\,1,187\,  &\,967    &~0  &\, 0.7  &~16   &\, 22   &\,593   &\,  3 &\,1.0 \rule{0pt}{2.8mm}\\ \hline
\,abp4pold         &\,L270\,&\,258 &\,2,547\,   &\,        &~0 &\,      &~      &\,      &\,       &\,    &\,    \rule{0pt}{2.8mm}\\ \hline
\,pdtvissfeistel   &\,L604\,&\,342 &\,2,111\,   &\,        &~0 &\,      &~      &\,      &\,       &\,     &\,    \rule{0pt}{2.8mm}\\ \hline
 \,kenflashp03     &\,L200\,&\,180 &\,14,943\,  &\,       &~0  &\,      &~      &\,      &\,      &\,    &\,    \rule{0pt}{2.8mm}\\ \hline
\,mentorbm1p00\,   &\,L8158\,&\,640&\,2.951\,   &\,         &~0 &\,     \,&~      &\,      &\,       &\,    &\,    \rule{0pt}{2.8mm}\\ \hline
%\,                 &\,    \,&\,    &\,     \,  &\,       &~0  &\,      &~      &\,      &\,      &\,    &\,    \rule{0pt}{2.8mm}\\ \hline
\end{tabular}                
\end{center}
\vspace{-5pt}
\label{tbl:flt_tst}
%\end{wraptable}
\end{table}
---------

%
%
%\vspace{-5pt}
\begin{table}
%\begin{wraptable}{l}{2.65in}
\small
\caption{\ti{Bug detection}}
\vspace{-5pt}
\scriptsize
\begin{center}
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
  \begin{tabular}{|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|@{}l@{}|} \hline
~name     &\,la- &\,\#inp\,&\,\#ga-   & \multicolumn{3}{c|}{random} & \multicolumn{5}{c|}{test generation}  \\
         &\,tch &\,vars\,&\,tes      & \multicolumn{3}{c|}{testing} & \multicolumn{5}{c|}{by \sas}  \\ \cline{5-12}
         &     &       &    &\,\#tests\,&\,\#cex\,     &\,time     &$|V|$&\,\#SSA\,&\,\#tests\,&\,\#cex\,&\,time\,  \\ 
&       &         &            &  &  &~(s.) & &   &   & &~(s.) \\ \hline
\,cmugigamax       &\,L124  &\,52  &\,1,003\,   &\,$10^7$ &~0  &\,143   &~29    &\,8,872 &\,1,001  &\,59 &\,0.9  \rule{0pt}{2.8mm} \\ \hline
\,kenoopp1         &\,L198  &\,81  &\,1,123\,  &\,$10^7$ &~0  &\,147   &~27    &\,5,256 &\,797    &\,111  &\,0.5 \rule{0pt}{2.8mm} \\ \hline
\,pd..blackjack4   &\,L120  &\,99  &\,625\,  &\,$10^7$ &~0  &\,36    &~25    &\,1,427 &\,314   &\,9   &\,0.8 \rule{0pt}{2.8mm}\\ \hline
\,abp4pold         &\,L270  &\,129 &\,1,177\,   &\,$10^7$  &~0 &\,293   &~28    &\,1,952 &\,1,893  &\,3   &\,1.2 \rule{0pt}{2.8mm}\\ \hline
\,pdtvissfeistel   &\,L604  &\,171 &\,1,055\,   &\,$10^7$  &~0 &\,355   &~22    &\,2,658 &\,1,505  &\,55   &\,1.0 \rule{0pt}{2.8mm}\\ \hline
\,mentorbm1p00\,   &\,L8670\,&\,626 &\,3,156\,   &\,$10^7$   &~0 &\,1,162\,&~27    &\,559   &\,175    &\,40  &\,2.5 \rule{0pt}{2.8mm}\\ \hline
\,139454p0         &\,L1676\,&\,791 &\,21,113\,&\,$10^7$   &~0 &\,679    &~19    &\,119   &\,115    &\,9   &\,169 \rule{0pt}{2.8mm}\\ \hline
%  &       &         &           &              & &                  &     &&   &   &   \\ \hline
\end{tabular}                
\end{center}
\vspace{-5pt}
\label{tbl:flt_tst}
%\end{wraptable}
\end{table}
--------
We consider the problem of finding a Complete Test Set (CTS) for a
combinational circuit $N$ that is a test set proving that $N \equiv
0$.  We use the machinery of stable sets of assignments to derive
non-trivial CTSs i.e. ones that do not include all possible input
assignments. The existence of non-trivial CTSs implies that it is more
natural to consider testing as structural rather than semantic
derivation (the former being derivation of a property that cannot be
expressed in terms of the truth table). Since computing a CTS for the
entire circuit $N$ is impractical, we present a procedure called \sas
that computes a CTS for a projection of $N$ on a subset of its
variables. The importance of \sas is twofold. First, it can be used
for generation of effective test sets.  Second, \sas can be used as a
starting point in designing verification tools that efficiently
combine structural and semantic derivations.
----------
As we mentioned earlier, the objective of applying a test to a circuit
is typically to check if the output assignment produced for this test
is correct. This notion of correctness usually means satisfying the
conjunction of \ti{many} properties of this circuit. For that reason,
one tries to spray tests uniformly in the space of all input
assignments.
-----------
Table~\ref{tbl:flt_tst} shows that tests extracted from CTSs for
projections of $N$ are very effective. This is not surprising taking
into account that formula relaxation employed in procedure
\ti{GenTests} (see Fig.~\ref{fig:gen_tests}) reminds stuck-at fault
testing. Note however a significant difference. Suppose that instead
of equivalence checking that is a ``global property'' involving
all circuit $N$, the latter specifies a \ti{local} property $\xi$ of circuit
$M$. In this case, only a very small part of $M$ is relevant to $\xi$.
So generating testing stuck-at faults of \ti{all the gates} of $M$
can be very expensive. Besides, the produced test set will contain
a lot of tests that are not relevant to $\xi$.
----------
%
%
%\vspace{-5pt}
\begin{table}
%\begin{wraptable}{l}{2.65in}
\small
\caption{\ti{Bug detection}}
\vspace{-5pt}
\scriptsize
\begin{center}
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
\begin{tabular}{|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{}l@{\,}|@{\,}l@{}|@{\,}l@{}|@{\,}l@{~}|@{~}l@{~}|} \hline
name     & la- & \#inp & \#ga-   & \multicolumn{2}{c|}{random} & \multicolumn{5}{c|}{test generation}  \\
         & tch &  vars   & tes      & \multicolumn{2}{c|}{testing} & \multicolumn{5}{c|}{by \sas}  \\ \cline{5-11}
         &       &         &            & \#tests       &  time     &$|V|$&\,\#SSA  & \#tests &\#cex &  time  \\ 
&       &         &            &$\times 10^6$&  (s.) & &   &   & & (s.) \\ \hline
cmugigamax       & L124  &  52  & 1,003   &  $>10$   &  143   &~29    &8,872 &1,001  & 59 & 0.9  \\ \hline
kenoopp1         & L198  &  81  & 1,123   &  $>10$   &  147   &~27    &5,256 &797    &111  & 0.5 \\ \hline
pd..blackjack4   & L120  &  99  & 625     &  $>10$   &  36    &~25    &1,427 & 314   &~9   & 0.8\\ \hline
abp4pold         & L270  &  129 & 1,178   &  $>10$   &  293   &~28    &1,952 &1,893  &~3   & 1.2\\ \hline
pdtvissfeistel   & L604  &  171 & 1,055   &  $>10$   &  355   &~22    &2,658 &1,505  &55   & 1.0\\ \hline
mentorbm1p00     & L8670 &  626 & 3,156   & $>10$    & 1,162  &~27    &559   &175    & 40  & 2.5 \\ \hline
139454p0         & L1676  & 791 & 21,113  & $>10$    & 679    &~19    &119   &115    & 9   & 169\\ \hline
%% pj2009  &  L1318 & 366     &  25,160   & mem &  $*$      &  $*$   &  $X$\,$\cup$\,$Y$    & 26 & 3.7 & 33 \\ \hline
%  &       &         &           &              &                   &     &&   &   &   \\ \hline
\end{tabular}                
\end{center}
\vspace{-5pt}
\label{tbl:flt_tst}
%\end{wraptable}
\end{table}
---------------
%
%
%\vspace{-5pt}
\begin{table}
%\begin{wraptable}{l}{2.65in}
\small
\caption{\ti{CTSs for circuits and their projections}}
\vspace{-5pt}
\scriptsize
\begin{center}
%\begni{tabular}{|p{22pt}|p{36pt}|c|c|c|c|} \hline
\begin{tabular}{|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{~}l@{~}|@{}l@{\,}|@{\,}l@{}|@{\,}l@{~}|@{~}l@{~}|} \hline
name     & la- & \#inp & \#ga-   & \multicolumn{3}{c|}{CTS for original } & \multicolumn{4}{c|}{CTS  for }  \\
         & tch &  vars   & tes      & \multicolumn{3}{c|}{circuit} & \multicolumn{4}{c|}{projection}  \\ \cline{5-11}
         &       &         &           & \#SSA         & \#tests       &  time     &\,proj.&\#proj.  & \#SSA   &  time  \\ 
&       &         &           & $\times 10^3$ &$\times 10^3$&  (s.) &\,type & vars  &$\times 10^3$    & (s.) \\ \hline
%visemodel  &  l30  &   13    &    54     &  54      &   1,544    & 0.1    & $~X$ & 13  & 102  & 0.0 \\ \hline
bob3 &  L26  &   14    &    41     &  46      &   2.0    & 0.1         & ~first  & 14  & 0.6    & 0.01  \\ \hline
eijks258   &  L10  &   16    &    45     &  259     &   8.2   & 0.5    & ~first  & 16  & 0.1   & 0.02 \\ \hline
%boblivear  &  L52  &   17    &    57     &  2,441   &  25,838    & 6.4      & $~X$  & 17  & 2,781 & 0.1 \\ \hline
cmudme1    &  L230 &   19    &    50     &  2,184   &  63   & 5.4     & ~first & 19  & 13 & 0.1 \\ \hline
mutexp0    &  L60  &   29    &    199    &  mem  &  $*$      &  $*$    &~first& 29  & 659 & 26 \\ \hline
pdtpmsmiim & L118  &   31    &    136    &  mem  &  $*$      &  $*$   & ~first & 31  & 936 & 4.2 \\ \hline
abp4pold   & L270  &  129    &    1,178  &  mem  &  $*$      &  $*$   & ~sec. & 25   &  2.2 & 0.4  \\ \hline
pj2009  &  L1318 & 366     &  25,160   & mem &  $*$      &  $*$   &  ~sec.  & 26 & 3.7 & 33 \\ \hline
mentorb..00  & L8670 &626 & 3,156     & mem &  $*$      &  $*$   & ~sec.    & 30 & 14 & 3.0 \\ \hline
139454p0& L1676  & 791     &  19,843   & mem &  $*$      &  $*$   & ~sec.   & 22  & 0.1  & 20 \\ \hline
%  &       &         &           &              &               &        &     &&      &  \\ \hline
\end{tabular}                
\end{center}
\vspace{-5pt}
\label{tbl:cts}
%\end{wraptable}
\end{table}
---------
\subsection{Choice of variables to project on}
\input{g4en_tests.fig}
Procedure \sas replaces computation of an SSA for formula $F_N \wedge
z$ with that of an SSA for a formula $H(V)$ where $V \subseteq \V{F_N
  \wedge z}$. Intutively, when choosing set $V$ one should use a
(small) coherent subset of variables reflecting structure and
semantics of $N$. One obvious choice of $V$ is the set $X$ of input
variables of $N$. In this case, an assignment of an SSA
for $H$ is also a test for circuit $N$. In general, however set $V$
contains internal variables of $F_N$, which makes generation of tests
from an SSA for $H$ a non-trivial task. In the following subsection, we
describe how it is done when $V$ forms an internal cut.
-------------------
Formula $H(V)$ can be viewed as describing \ti{a projection of
    circuit} $N$ on $V$. So, $T$ can be viewed as an
  \ti{approximation} of a CTS for circuit $N$. If $V$ is the set $X$
  of input variables, then an SSA found by \sas for $H(V)$ is itself a
  test set. In section~\ref{sec:int_cut}, we describe generation of a
  tests set when $V$ contains internal variables of $N$.
  ----------------
\footnote{If set $X$ is too large, one can use a
  ``piece-wise'' construction of tests as described
  in~\cite{cmpl_tst}. In this case, one partitions $X$ into subsets
  $X_1,\dots,X_k$ of manageable size and computes projections of $N$
  on $X_i$,$i=1,..,k$.}
  --------------------
In particular, we describe a
procedure for ``piecewise'' construction of tests that can be
potentially applied to very large circuits.
---------------
Table~\ref{tbl:flt_tst} shows that tests extracted from CTSs for
projections of $N$ are very effective. The fact that these tests are
effective even for strategy 2 is very encouraging for the following
reason. Computing a CTS for a projection $N^V$ where $V$ is small is
close to regular SAT-solving. (They become identical if $V =
\emptyset$.) Thus, by breaking $X$ into relatively small subsets
$X_1,\dots,X_k$ and using piecewise construction of tests as described
above, one will get an effective test set that can be efficiently
computed even for very large circuits.
-----------
To generate $T$ we used two strategies. In strategy 1, $T$ was
generated as a CTS for projection $N^X$. Strategy 2 was employed when
\sas failed to build a CTS for $N^X$ due to memory overflow or
exceeding a time limit.  In this case, we partitioned $X$ into subsets
$X_1,\dots,X_k$ and computed sets $T_1,\dots,T_k$ where $T_i$ is a CTS
for projection $N^{X_i}$. (In the examples where we used strategy 2,
the value of $k$ was 2 or 3). The Cartesian product $T_1 \times \dots
\times T_k$ forms a test set for $N$.  Instead of building the entire
set $T$, we randomly generated tests of $T$ one by one as follows.
The next test \pnt{x} of $T$ to try was formed by taking the union of
$\pnt{x}_i$,$i=1,\dots,k$ randomly picked from corresponding
$T_i$,$i=1,\dots,k$. Note that in the extreme case where every $X_i$
consists of one variable, strategy 2 reduces to generation of random
tests. Indeed, let $X_i=\s{x_i}$,$i=1,\dots,k$ where $k = |X|$.  Then
formula $H(X_i)$ for projection $N^{X_i}$ is equal to $x_i \wedge
\overline{x}_i$. The only SSA for $H(X_i)$ is trivial and consists of
assignments $x_i=0$ and $x_i=1$ (and so does $T_i$). By randomly
choosing a test of $T_i$ one simply randomly assigns 0 or 1 to $x_i$.
---------------
In this section, we describe results of two experiments. In the first
experiment (Subsection ~\ref{ssec:cts}), we computed CTSs for circuits
and their projections.  In the second
experiment(Subsection~\ref{ssec:bug}), we used \sas for bug
detection. In particular, in Subsection~\ref{ssec:bug}, we describe a
method for ``piecewise'' construction of tests. Importantly, this
method has the potential of being as scalable as SAT-solving and hence
to be used to generate high-quality tests for very large circuits.  In
both experiments we used miters i.e. circuits specifying the property
of equivalence checking. (The miter shown in
Figure~\ref{fig:gen_miter} evaluates to 1 for an input assignment
\pnt{x} iff the output values of $M'$ and $M''$ are different under
\pnt{x}.)  We also experimented with circuits specifying other
properties. For the lack of space we omit a description of those
experiments.
----------------
Ideally, it would be nice to have an option of generating a test set
where the ratio of assignments for which $K$ evaluates to 1 is higher
than in the truth table of $K$.  One can achieve this objective as
follows.
---------
\footnote{One can give a more
  precise explanation of when and why using $T_K$ should work.}
  ---------------
Let $M^*$ be a circuit obtained by modification of $M$. Suppose that
one needs to check whether $M^*$ is still correct. This can be done by
checking if $M^*$ is logically equivalent to $M$. However, equivalence
checking cannot be used if the functionality of $M^*$ has been
intentionally modified. Another option is to run a test set previously
generated for $M$ to verify $M^*$. Generation of CTSs can be used to
empower this option. The idea here is to re-use CTSs generated for
testing the properties of $M$ that should hold for $M^*$ as well.



Let $\xi$ be a property of $M$ that is supposed to be true for $M^*$
too.  Let $N$ be a single-output circuit specifying $\xi$ for $M$ and
$T$ be a CTS constructed to check if $N \equiv 0$. To verify if $\xi$
holds for $M^*$, one just needs to apply $T$ to circuit $N^*$
specifying property $\xi$ in $M^*$. Of course, the fact that $N^*$
evaluates to 0 for the tests of $T$ does not mean that $\xi$ holds for
$M^*$. Nevertheless, since $T$ is specifically generated for $\xi$,
there is a good chance that a test of $T$ will break $\xi$ if $M^*$ is
buggy. In Subsection~\ref{ssec:bug}, we substantiate this intuition
experimentally.
-----------
Let $M$ be a multi-output combinational circuit.  In this section, we
consider some applications of \sas to testing $M$. They can be used in
two scenarios.  The first scenario is as follows.  Let $\xi$ be a
property of $M$ specified by a single-output circuit $N$. Consider the
case where $\xi$ can be proved by a SAT-solver. If one needs to check
$\xi$ only once, using the current version of \sas does not make much
sense (it is slower than a SAT-solver). Assume however that one
frequently modifies $M$ and needs to check that property $\xi$ still
holds.  Then one can apply \sas to generate a CTS for a projection of
$N$ and then re-use this CTS as a high-quality test set every time
circuit $M$ is modified (Subsection~\ref{ssec:des_changes}).

The second scenario is as follows. Assume that some properties of $M$
cannot be solved by a SAT-solver and/or one needs to verify the
correctness of circuit $M$ ``as a whole''. (In the latter case, a
SAT-solver is typically used to construct tests generating events
required by a coverage metric.) Then tests generated by \sas can be
used, for instance, to hit corner cases more often
(Subsection~\ref{ssec:corners}).
----------------
Formula $H$ produced when $G$ is unsatisfiable is logically
  equivalent to \prob{W}{G}. Thus, \sas can be viewed as a quantifier
  elimination algorithm for unsatisfiable formulas. On the other hand,
  \sas can be applied to check satisfiability of a CNF formula, which
  makes it a SAT-algorithm.
  -------------------------
The notion of non-trivial CTSs helps better understand testing.  The
  latter is usually considered as an incomplete version of a
  \ti{semantic derivation}. By semantic derivation we mean proving a
  semantic property of a circuit or formula i.e one that can be
  expressed in terms of the truth table. This point of view explains
  why testing is efficient (because it is incomplete) but does not
  explain why it is effective (only a minuscule part of the truth
  table is sampled). As we show later, a non-trivial CTS is a
  structural property of $N$. That is, the fact that a set of tests
  forms a non-trivial CTS cannot be expressed in terms of the truth
  table of $N$. For that reason, a non-trivial CTS is
  circuit-specific. So it is more appropriate to consider testing as a
  version of a \ti{structural derivation} (possibly incomplete). This
  point of view explains not only efficiency of testing but provides a
  better explanation for its effectiveness: by using circuit-specific
  tests one can cover a significant part of a non-trivial CTS.
----------  
\subsection{Property-specific testing}
\label{ssec:pspec_test}
Let $M$ be a multi-output combinational circuit. Typically, testing is
used to check if the output assignment produced by $M$ for some input
assignment displays an incorrect behavior. Thus, testing is employed
%
\input{c2ut.fig}
%
to verify \ti{many} properties at once. For that reason, usually one
generates a set of tests that is uniformly distributed in the space of
all input assignments.  However, uniform distribution may not be the
most effective way to verify a \ti{particular} property.


\sas can be used to generate \ti{property specific} tests. Let circuit
$N$ specify a property $\xi$ of $M$.  Suppose that \sas is efficient
enough to generate a CTS for a projection of $N$ thus proving $\xi$
true. Just showing that $\xi$ holds does not make much sense if \sas
takes more time than a SAT-solver solving $F_N \wedge z$.  However, in
contrast to a resolution proof, a test set $T$ built by \sas can be
easily \ti{re-used} to check if $\xi$ still holds for a modified
circuit $M^*$.  One just needs to apply $T$ to circuit $N^*$
specifying property $\xi$ for $M^*$.  Of course, the fact that $N^*$
evaluates to 0 for the tests of $T$ does not mean that $\xi$ holds for
$M^*$. Nevertheless, since $T$ is specifically generated for $\xi$,
there is a good chance that a test of $T$ will break $\xi$ if $M^*$ is
buggy. In Subsection~\ref{ssec:bug}, we experimentally substantiate
this intuition.

\subsection{Using CTSs of easy properties to direct testing}

Suppose that generation of a CTS for a projection of $N$ is too hard
for \sas. (We assume again that $N$ specifies a property $\xi$ of
circuit $M$.) Besides, $F_N \wedge z$ is too hard for a SAT-solver.
In this case, one can try to generate CTSs for weaker properties that
are relevant to $\xi$ e.g. ones implied by $\xi$. Suppose, for
instance, that $R$ is a cut of $N$ (see Figure~\ref{fig:cut}) and
\pnt{r} is an assignment to $R$ under which $N$ evaluates to 1. Let
$\xi^*$ denote the property that for every input assignment of $N$,
the assignment to $R$ produced by $N$ is different from \pnt{r}. Then
one can use a test set $T$ generated by \sas when proving $\xi^*$ to
test property $\xi$.


%\subsection{Taking care of structural peculiarities}
----------
\tb{\scriptsize{1}}\> $G^* := G \setminus \mi{SatClauses}(G,\pnt{v})$\\
\tb{\scriptsize{2}}\> $U := \emptyset$ \\
\tb{\scriptsize{3}}\> while ($|U| < |W|$) \{ \\
\tb{\scriptsize{4}}\Tt  $(\pnt{p},R) := \mi{CheckSat}(G^* \wedge U)$\\
\tb{\scriptsize{5}}\Tt if ($\pnt{p} = \mi{nil}$)  return($\overline{U},\mi{nil}$)\\
\tb{\scriptsize{6}}\Tt $w_i := \mi{PickVar}(\pnt{w} \setminus \pnt{p})$ \\
\tb{\scriptsize{7}}\Tt if ($w_i = \mi{nil}$) return($\mi{nil},\pnt{p}$)\\
\tb{\scriptsize{8}}\Tt $U := U \cup \s{\mi{UnitCls}(w_i,\pnt{p})}$ \}\} \\
--------------------------
$\mi{SemStr}(G(V,W))$\{\\
\tb{\scriptsize{1}}\> $H := \emptyset$ \\
\tb{\scriptsize{2}}\> while (\ti{true}) \{ \\
\tb{\scriptsize{3}}\Tt $(\pnt{v},P,\sub{p}{init},\Fi) := \mi{BldSSA}(H)$\\
\tb{\scriptsize{4}}\Tt if ($P \neq \mi{nil}$)  \\
\tb{\scriptsize{5}}\ttt return($H,\mi{nil},P,\sub{p}{init},\Fi$)\\
\tb{\scriptsize{6}}\Tt  $(C,\pnt{p}) := \mi{GenClause}(G,\pnt{v})$ \\
\tb{\scriptsize{7}}\Tt  if ($\pnt{p} \neq \mi{nil}$) \\
\tb{\scriptsize{8}}\ttt return($\mi{nil},\pnt{p},\mi{nil},\mi{nil},\mi{nil}$)\\
\tb{\scriptsize{9}}\Tt  $H := H \wedge C$ \} \\
-------------
Assume that $F$ is a CNF formula. (We will use this assumption for all
the formulas considered in this paper.) An example of the structural
property is the redundancy of a clause $C$ in $F$. Indeed, suppose that
formulas $F$ and $G$ contain clause $C$ and $F \equiv G$. The fact
that $C$ is implied by $F \setminus \s{C}$ does not mean that $C$ is
implied $G \setminus \s{C}$. An example of a semantic property is an
implication. If $C$ is implied by $F$ and $F \equiv G$, then $C$ is
implied by $G$ as well.

--------------------

An example of a semantic property is implication. If $C$ is implied by
$F$ and $F \equiv G$, then $C$ is implied by $G$ as well. An
interpolant is an example of a structural property.  Suppose that
$J(Y)$ is an interpolant for formula $A(X,Y) \wedge B(Y,Z)$ i.e.  $A
\rightarrow I$ and $I \rightarrow \overline{B}$.  Formula $J$ may not
be an interpolant for $A'(X,Y) \wedge B'(Y,Z)$ logically equivalent to
$A \wedge B$ if, for instance, $A \not\equiv A'$ and/or $B \not\equiv
B'$.

-----
Let us consider the challenges of purely semantic derivation by the
example of propositional SAT-solvers based on resolution. Since the
resolvent clauses produced by resolution are implied by the original
formula, such SAT-solvers perform semantic derivation. Suppose one
needs to solve formula $A(X,Y) \wedge B(Y,Z)$ where $X,Y,Z$ are sets
of Boolean variables. Assume also that set $Y$ is much smaller than
$X$ and $Y$. So one can view formula $A \wedge B$ as describing two
blocks ``communicating'' via variables of $Y$. Modern SAT-solvers are
based on derivation of conflict clauses. Typically, such a SAT-solver
starts deriving clauses relating internal variables of blocks $A$ and
$B$ thus losing the two-block structure of the original
formula\footnote{\input{f2ootnote}}.
------
 The satisfiability of $F_N \wedge z$
is typically checked by a resolution-based SAT-solver.
Every clause produced by resolution is implied by the original
formula. Since implication is a semantic property, this method of
solving Circuit-SAT can be viewed as semantic.
----------
We will call $T$ a trivial CTS if it consists of all $2^{|X|}$ tests.
A traditional point of view is that the only CTS for $N$ is the
trivial one. In other words, one considers testing just as sampling
the truth table of circuit $N$ that ignores its specifics.  A flaw of
this point of view does not explain why testing is so effective taking
into account that only a minuscule part of the truth table is sampled.
The existence of non-trivial CTS provides at least two reasons for
such effectiveness. First, the size of a CTS can be much smaller than
$2^{|X|}$. Second, a CTS is circuit specific. (This is due to the fact
that, as we show in Section, an SSP is formula specific. The fact that
$P$ is an SSP for formula $H$ does not mean that it is also an SSP for
a formula $Q$ logically equialent to $H$.) This means that a good set
of tests exploits the structure of circuit $N$ (which is quite obvious
for an experienced verification engineer). 
-----------
This algorithm accepts formula $F$ that is satisfiable iff $N
  \not\equiv 0$. It outputs a) formula $F^*$ logically equivalent to
  $F$ that depends only on variables of $X$ and b) a set of
  assignments to $X$ forming an SSP for $F^*$. The existence of an SSP
  for $F^*$ means that the latter is unsatisfiable and hence $N \equiv
  0$ holds.
----------
 A straightforward way to build an CTS is to generate
an SSP $P$ of $F_N \wedge z$ and then form the set of the tests
specified by points of $P$. (A point $\pnt{p} = (\pnt{x},\pnt{y},z)$
of $P$ specifies test \pnt{x}).
----------
Then
\pnt{s} can be reached from \pnt{p} by the following procedure
building a sequence of points $\ppnt{p}{1},\dots,\ppnt{p}{i}$ where
\ppnt{p}{1} = \pnt{p}. Pick the current assignment \ppnt{p}{i} (originally
$i=1$).  If \ppnt{p}{i} = \pnt{s}, then \pnt{s} is reached. Otheriwse,
an arbitrary clause $C$ of $H$ falsified by \ppnt{p}{i} is chosen. Since
\pnt{s} satisfies $C$, there is a variable $v$ such that $v \in \V{C}$
and assignments to $v$ are different in \ppnt{p}{i} and
\pnt{s}. Generate point \ppnt{p}{i+1} obtained from \ppnt{p}{i} by
flipping the value of $v$ and make \ppnt{p}{i+1} the current
assignment.
----------
 Only one assignment of \cube{x}{i} specifies the
correct execution trace for test \ppnt{x}{i} i.e. one produced by $N$
under input \ppnt{x}{i}.  All the other assignments specify erroneous
traces. 

